CodeAid: Evaluating a Classroom Deployment of an LLM-based Programming Assistant that Balances Student and Educator Needs

Timely, personalized feedback is essential for students learning programming. LLM-powered tools like ChatGPT offer instant support, but reveal direct answers with code, which may hinder deep conceptual engagement. We developed CodeAid, an LLM-powered programming assistant delivering helpful, technically correct responses, without revealing code solutions. CodeAid answers conceptual questions, generates pseudo-code with line-by-line explanations, and annotates student's incorrect code with fix suggestions. We deployed CodeAid in a programming class of 700 students for a 12-week semester. A thematic analysis of 8,000 usages of CodeAid was performed, further enriched by weekly surveys, and 22 student interviews. We then interviewed eight programming educators to gain further insights. Our findings reveal four design considerations for future educational AI assistants: D1) exploiting AI's unique benefits; D2) simplifying query formulation while promoting cognitive engagement; D3) avoiding direct responses while encouraging motivated learning; and D4) maintaining transparency and control for students to asses and steer AI responses.

==> sections/temp.tex <==
\section{9 - Discussion}

To increase the accuracy and helpfulness of some features, particularly the complex features we need to improve transparency of what the 'unpredictable black-box AI' is doing and provide ways to direct it.
As the complexity of features increases, so does the challenge of steering the AI for accurate and helpful responses. The \textit{Help Fix Code} feature in CodeAid, which required performing a complex series of steps~\ref{redesigned_help_fix_code}, Although students really liked the ability to have their code annotated by the AI, it sometimes produced incorrect or unhelpful responses, especially with complex code. 
We can think of several reasons for this,
- the input token limitations (students were not able to paste in their entire code)... which were a limitation of the OpenAI models we were using back then.
- not being able to handle multiple files, relevant context that is being used in the code, assumptions about the task... which would still exist even if we developed code editor plugins that had access to the entire project.
- the complexity and hidden (blackboxed) algorithm and process for displaying the response which made it difficult to understand "why the AI is suggesting some fix"

our results showed that students did not like when the AI was too confident about an output that it generated which was incorrect. These LLMs (especially after going through the RLHF process) are making a lot of assumptions and guesses which may not be true for the user's particular use-case. Future tools should be transparent about what the AI is "guessing" about, instead of being too confident with their response. For example, future tools can query the user about what the AI does not know about the context and what is missing from the code that they've provided. This increases transparency, and allows users to understand the AI's logic and iteratively refine hte output to lead to more accruate results and hopefully deeper learning. By Incorporating HCI methods like progressive disclosure \cite{nielsen2006progressive} future tools can allow the user to be "in the loop" and enable the user to steer the AI instead of it \textit{guessing} a response that could potentially be incorrect due to the incorrect assumptions.


% ---------–---------–---------–---------–---------–

The main interactions regarding how easy it could be when using such an AI coding assistant are (i) how they provide input, (ii) the cognitive load associated with selecting (and potentially predicting the output and whether its output will be useful for them in their scenario or not) and deciding which feature to use for their problem, and (iii) how they can steer the model and deal with the AI's inaccuracies and unhelpful responses (or whether they can ask the question differently).

\subsubsection{How to provide input and select from available features}
CodeAid required students to first select a feature, type a prompt using the two input boxes (one for code and one for the message -- in which the purpose and meaning of the input boxes changed when different features were selected), and then hit the generate button. This was because of the way we implemented the LLM function and rendering components in which each feature was designed to be completely separate from each other. Additionally, we found that for some use-cases, students used a variety of different features. Given the varying themes in the questions that students asked (four major categories and nine sub-categories), the system's output should be based on "what students are asking" and "what they want" rather than the feature they selected. Additionally, We found that when students used CodeAid, they used a variety of features, in different ways when they wanted to do something (let's say debug code). sometimes they used the \textit{General Question} to understand the error message, the \textit{Question from Code} to understand what something is doing, and the Help Fix Code to help them identify the problems in their code. Since this selection might have been cognitively difficult. -- although educators thought that thinking before selection process was a good interface as it helped students think before using the tool, but students found it difficult and preferred ChatGPT's free-form editing. -- As a solution, future tools can provide a free-form text editor as input with optional and simple syntax highlighting such as MarkDown, and use an intermediary LLM function that would suggest the most relevant features of the system for the given input prompt. The LLM then provides the appropriate inputs for each of those features and students can then simply select any of those features, or even try them all.

- then an LLM (similar to function calling API) will show the top most relevant features of the system for the user to decide and pick from. They will have the freedom to use all of them if they make sense. so for example if they're asking to help debug some code, a student might want to paste their code from two files, the error message their getting, and the expected output, then the system produces a variety of responses for them to chose based on their question: highlight the potentially incorrect parts of their code, explain with examples and documentations of some of the functions or patterns that they're using, and 


Input length and Handling Multiple files:
One of the issues students had with CodeAid compared to ChatGPT was CodeAid's lower token input (which was a limitation of our tool) and that they were not able to provide their entire project files, future tools should also be developed that can "see" their entire project, not just one file. there might be some UX design challenges here. One solution is to develop such tools as plugins for code editors. However, making such educational tools too accessible might increase the frequency of access (due to proximity) and create over-reliance, however, this can potentially be fixed by using levels of scaffolding that enable deeper cognitive engagement with their programming problem, or using throttling (to disable a feature after using it too frequently).

\subsubsection{How to provide better steering capabilities}
As features become more complicated, they were more difficult to steer so that students could iterate with in order to get more accurate responses. For example, the \textit{Help Fix Code} feature was designed to tell which lines of code are incorrect, what code is missing and etc. The feature required three serial functions (one for generating the correct code, one for annotating the diff, and one for adding LLM annotations). From our thematic analysis, we found that the feature was incorrect and unhelpful in many cases, particularly as the code become more complex. 
In these cases, it is very important to provide ways for the user to know "why" the model is producing its current output (e.g. the user to understand its underlying assumptions about the provided code) and allow the user to edit and provide more info. As a way to not overwhelm the student with a ton of information, this extra information could be minimized at first and only displayed if the student wants to "debug" and steer the model when it had inaccuracies. 

Overall, future systems should provide more transparency (e.g. by displaying the assumptions that the AI is making) and more steerability (e.g. by asking the user to verify those assumptions, or provide some of the unknown parts like function definitions that are being used in a provided code etc in an interactive way, similar to HCI methods like progressive disclosure \cite{nielsen2006progressive}) 

% Future tools should also explain the guardrails that are in place, for example if the student asks for code implementation for part of their assignments or projects, then it should tell them that it's "I'm not able to generate the code, but here are some options I can help you with"



------------------------


Designing LLM-Powered tools for educational settings require balancing multiple dimensions like ease of use, being correct and helpful but in a way that pedagogical and ethical considerations
promotes deep engagement, while being more valueable compared to alternatives that do not have guardrails. This is a complicated task, however, CodeAid's iterative development, results from its semester-long deployment, and the educator interviews can pave the way for future LLM-Powered Coding Assistants for educational settings. In summary, future tools should:

- provide non-AI fall-backs when accuracy might be low (such as when trying to help with debugging, the least accurate feature of our system)
- provide verifiable resources and enable self-verification

- allow for customization for different scenarios and use-cases, picking from different scaffolding methods, last resorts

- and eventually, be easy to use (given the complexity of interacting with a blackbox AI model) in terms of providing input, what to expect and predict, and how to steer the AI
    - be transparent: show assumptions, performance history, 
    accuracy, correctness, and helpfulness (so the user does not need to trial-and-error) and be easy to steer and 
    - be easy to navigate
    


From a high-level we can see that educators wanted students to stay in AI tools that were designed with guardrails (knowing that there's a learner using it compared to someone that just wants to maximize productivity). From our end-of-semester survey comparing students' usage of CodeAid with ChatGPT, we found that this requires: ease of use for inputs and steering, course-specific features that provide an added value, higher accuracy, and interactive features.

Future tools also need to provide a variety of scaffolding and 


Features like General Question and Explain Code were overall more successful, and similarly usages like Asking Programming Questions, Writing and Explaining Code were more accurate, helpful, and received better feedback. However, one of the main use cases with Debugging Code was less accurate, less helpful, and received lower ratings.







\textbf{Course-Specific Tools:}
CodeAid was designed to be more general-purpose and help students with any C programming task, but 
- when answering questions, pull information directly from lecture notes and examples that were covered in the curriculum. similar to the relevant function documentation that students liked in CodeAid.
- link to instructor-verified material from the class
- AI that can answer questions about assignments and projects


\textbf{Improved Trust and Reliability:}
- each of the suggested features can have a "confidence level" associated to them at two levels: based on the students' query, display what are the unknown assumptions about each method (e.g. if a feature is just prompting them to think about things, then the unknown assumptions are less compared to another feature that is trying to fix the student's code without knowing their entire codebase)
- if course-specific tools are developed, then the automatic feature suggestion system can also detect which project/assignment students are asking about, and then directing their query to a specific query that knows about that particular project or assignment. as a way to improve accuracy, similar to a TA that is able to better help when they know the solution, they can not only identify what's wrong in a student's code but also provide good hints to them. (below we will talk about the amount of scaffolding and directness) The system is then able to provide scaffolded ways of helping them with much higher accuracy since it has access to the instructor-verified solution, but because of the guardrails, it will never reveal it to the students directly.

\textbf{Interactive Features:}
Students showed many positive feedback regarding the interactive features developed in CodeAid compared to ChatGPT. they liked the line-by-line explanations, the interactive pseudo-code, highlighting erronous lines of code, and the summarized relevant function documentations. Future tools should expand on these features and make them more interactive as a way to improve deeper engagement. A repository of different assistance types, line-by-line code execution similar to PythonTutor, scaffolded hierarchical methods of showing code.


% - our results from a real-world deployment show that (1) the majority of students and their queries were not asking for direct code solutions, and (2) many students found the system helpful (although some features were better) and they continued using CodeAid's even though it produced indirect responses 


\textbf{How Direct should Future tools be?}
- CodeAid only provided one type of directness for all: pseudo-code. Although it helped students think, but future tools can provide different levels of directness.
- we found that in the first half of the semester, students did not like that the system does not produce any code at all, that was fixed in our second iteration with the relevant function documentation. our thematic analysis also revealed the types of questions that students asked, in which not all of them have been directly asking for code solutions and that students that used ChatGPT reported that they liked that it produced code examples. Therefore, future tools can differentiate between example and direct code solutions:
students liked that ChatGPT generated example codes, and prior research has showed that programmers learn from example codes.
- future tools can (and should) provide code examples since many students learn from 
- this could potentially keep students in these tools instead of defaulting to ChatGPT


For more complex usages like debugging, which was one of the main usages of CodeAid, we found that both the first and second iteration of the help-fix-code had low accuracy.





\textbf{Provide Varying levels of scaffolding}
- varying levels of directness: less direct when students copy task descriptions or directly ask for specific code implementations, compared to when they're asking for what some function does vs. how they can implement this behavior using X vs. how they can use something vs. .even those that reported using ChatGPT, reported that the direct responses generated by ChatGPT were not good for learning. 
- Since some students have strong preferences (e.g. having a personal desirie for self-reliance and solving tasks by themselves) then the system can have some pedagogical settings and customization fields to control: do they want to come up with the solutions themselves, vs. be more direct.
- provide the skeleton of the code, but them fill in the important parts themselves, or help them by asking problem solving questions so that they can come up with the solution themselves.


\textbf{Provide Non-AI alternatives:}
- some students reported that they lost trust in CodeAid after it did not respond correctly. Future systems that want to still maintain high can include some "last-resort"
- Provide non-AI alternatives: ask question from professor (as email), ask on Q/A forum, etc. (so the AI first suggests: try these before contacting the professor)
- help them fix their code themselves by providing debugging strategies and suggestions based on their current status and code.





Our v2 system enabled many interactive features in response to students' requests from the first half of the study, however, given the complex nature of how they were implemented with the OpenAI APIs that were available at the time, they required multiple serial LLM calls, which reduced their steerability and transparency (e.g. the user is very limited in terms of how they can steer and navigate the model for example when it has some missing assumptions or something else).

Future tools, can utilize the powerful capabilities of GPT-4 that follows provided templates to create domain-specific languages (DSLs) \cite{ym2023pwr} be designed with GPT-4's DSL support and report back any "guesses" that they're making and assumptions that they're having when.





\textbf{Interactive Features}


\textbf{Contextual Relevance:}
It seems that the more students feel like this tool was specifically designed and tailored to their class (compared to being something generic) it becomes more useful to them.
Future tools should provide assistance on projects, assignments, (e.g. helping students with their misunderstandings about the project).


One concern is whether they will show code solutions, and our results show that with proper prompt engineering and analytic dashboards, this will not be a problem.

Our results showed that guardrails can be trusted and when designed properly, can still be engaging and helpful.

work, and now with GPT-4, which provides more controllability over the context of the LLMs output, we are able to build these tools with more confidence and less concern about them showing the code solution.


This is the most certain thing that we learned -- it optimizes multiple things:

- makes sure that responses are in students' zone of proximal development, increasing learning effectiveness
- promotes self-verification, so students
- it helps students stay in these "approved" tools that have these "guardrails" instead of defaulting to ChatGPT
-  


- providing more course-specific material
- general purpose vs. specific class
general-purpose vs. specific for class
our results are a bit more in favor of specific for class. help keep students away from chatgpt, better and more targeted responses, and allows students to ask about project/assignments

we have evidence from the interviews and weekly surveys that show how students liked and felt that the tool is targeted more towards C programming compared to ChatGPT and other tools... so future tools: the more students understand that the tool is tailored specifically to their course, their assignments, their projects, they will use it more for the class.
- ask about projects/assignments
[any other ways to attract students to keep in the tool?]




Pedagogical:
Provide Varying levels of scaffolding

Educators' emphasis on pedagogical soundness (RQ4) suggest that future tools should promote deeper cognitive processing. 

The variability in students' usage patterns (RQ1) the need for adaptive strategies, resonating with the constructivist theory of learning with posits that knowledge is actively constructed by the learner based on their experiences and interactions.

- Scaffolding method: promote critical thinking, problem-solving, and self-reflection.



Contextual Assistance:
- 

Contextual Relevance:
- 



Response Accuracy and Trust:
- 






Our results from deploying CodeAid 
- understand how students will use such a tool in a semester-long deployment, what types of questions they will ask, how they use this tool in comparison to other available tools that they have (office hours), and what new unique interactions and usages it will enable. whether it will help scale up instruction and help under-represented groups?
- we then tried to understand what did students think of the LLM's responses? and how did we (the researchers) evaluate the responses in terms of correctness, helpfulness, and directly revealing code solutions. we frequently asked students why they used or not used the system, and how it helped them?
- at the end of the course, we asked students to compare CodeAid with ChatGPT. This helped us see which parts of our results could be generalized, which parts are related to the interaction, and where did CodeAid do better, and where did ChatGPT do better.
- Finally, we conducted eight interviews with educators that serves as a great bridge from CodeAid to beyond CodeAid and the implications for future LLM-powered coding assistants.
- This section aims to extend the discussion beyond CodeAid, using our findings as a foundation to inform the design of future LLM-Powered Coding Assistants specifically tailored for learning environments.

% A summary of what we found:
Our semester-long deployment of CodeAid 
- our thematic analysis of ~1750 queries asked from CodeAid using the five features that we developed, helped us identify four categories and nine subcategories of different types of queries and their frequency/proportions.
- we found that 79\% of responses were correct, and 67\% were helpful. We also identified reasons for when students rated queries high or poorly for each of the features. In terms of directly revealing code solutions, X\% were only in natural language, Y\% included high-level pseudocode, Z\% included specific pseudocode, N\% included 
- support for under-represented groups: females used the system more compared to males, and 
- 

------------------------------------------------------------------------------------------------------------



adapting to learner's zone of proximal development (Vygotsky’s):
- LLMs can act as a more knowledgeable other... adaptive responses cater to individual learning needs... some students wanted to explain things "like an eight year old" or they really liked how they could ask many questions without being judged... 

Promoting Critical Thinking... ask probing questions or offer guidance that leads students to discover solutions themselves, rather than providing direct answers.

constructivist learning principles, where knowledge is actively constructed by the learner... aligning with Piaget’s theory of cognitive development.

% The variability in students' usage patterns (RQ1) underscores the need for adaptive learning strategies, resonating with the constructivist theory of learning which posits that knowledge is actively constructed by the learner based on their experiences and interactions (Piaget, 1954). Future LLM-powered tools should personalize learning paths, adapting to individual student's inquiry types and frequencies, thereby facilitating a more tailored and effective learning experience. This aligns with Vygotsky's (1978) zone of proximal development, suggesting that tools should provide scaffolding adjusted to the learner's current level of understanding.


% \subsubsection{Enhanced Pedagogical Approach}
% Educators' emphasis on pedagogical soundness (RQ4) suggests that future tools should not only offer correct responses but also promote deeper cognitive processing. This aligns with Mayer’s Cognitive Theory of Multimedia Learning, which advocates for designing educational experiences that optimize cognitive processing. Tools should encourage critical thinking and problem-solving skills, reflecting Bloom's Taxonomy, by guiding students through the problem-solving process rather than providing direct solutions.


% \subsubsection{Student Engagement and Interactive Learning}
% The request for more interactive features like code execution (RQ4) and high usage of interactive features in CodeAid (RQ1) point towards the need for more engaging and interactive learning experiences. According to Malone's Theory of Intrinsically Motivating Instruction, such features can enhance curiosity and control, key elements for engaging learning experiences. Interactive exercises, aligned with experiential learning theory (Kolb, 1984), can provide hands-on learning opportunities, enhancing understanding and retention.


% \subsubsection{Customization and Control for Educators}
% Educators' desire for customizable responses (RQ4) suggests that future tools should allow instructors to tailor the tool’s behavior to align with their pedagogical goals and course content. This is consistent with the concept of Technological Pedagogical Content Knowledge (TPACK), which emphasizes the intersection of technology, pedagogy, and content in effective teaching. Educators should be able to configure the tool to vary the level of guidance based on the course level and learning objectives.


% \subsubsection{Monitoring and Analytics}
% The suggestion for monitoring dashboards (RQ4) aligns with the need for formative assessment tools in education, as posited by Black and Wiliam (1998). These dashboards can provide educators with insights into student learning processes, helping identify common misunderstandings and adjust teaching strategies accordingly. However, this should be balanced with considerations of privacy and student autonomy.



different levels of optimization:
students liked the interactive features of CodeAid, such as the line-by-line explanations of the pseudocode. however, both educators and students found 
- direct vs. indirect -> dynamically deciding: code vs. pseudocode vs. some other indirect method (e.g. making the user think about the task) (Differentiating Between Examples and Solutions)



Single Text Input with AI-Suggested Responses and Alternatives:
- ease of use and learning? In comparison to ChatGPT, students wanted an easier way to interact with the system.... interactive features of CodeAid were fine... the problem was with how they needed to specify the action and do many clicks. so future tools should 


our results, including the dataset of questions asked by students that we made public, help develop future tools by understanding what types of questions students asked. which means we 

- if they didn't like the responses, then it should provide alternatives. this could also reduce the chance of switching to unguraded tools like ChatGPT

similar to bing chat's references, CodeAid's relevant function documentations was highly favored by the students from our deployment. future tools can improve this for several reasons:
- improved self-verification
- provide more learning opportunities
this can also be extended by tools similar to Bing Chat that provide sources from around the web (e.g. w3schools, wikipedia, etc.)


Reasons to Keep Students in the tool:


if a student does not trust codeaid, provide prompt builders, so that they'd at least have the chance to use chatgpt with guardrails... guardrails that they could edit themselves if needed.

Future tools should be designed to provide various AI and non-AI alternatives
non-AI can be:
- using the LLM to convert the student's question to a proper Stackoverflow question so they can ask there, or something that they can post on the Q/A forum of their class


% excited about AI: scaling up instruction + mimicing what an expert instructor would do
% Expected general design guidelines for the design of classroom tools using LLMs -> people designing classroom tools using LLMs 
% general design principles for LLM-based coding tools
% broader insights” that inform the design of LLM-powered coding assistants
% critical discussion of how answers to set RQs could have an impact on future design and adoption of digital TA  
% Is it possible to make a system that optimizes for both learning and ease-of-use? Or is this a fundamental tradeoff in the design of LLM-based educational tools?


Unlike CodeAid that provided similar levels of directness to all queries, future tools should be able to provide a customized 



Future classroom assistants should provide different levels of directness for different types of asked queries.
If students request for direct code solutions (which was 10\% of the questions asked), the system should work as a guiding TA. At first asking self-reflecting questions so they can think more deeply about the task and if that was not enough, allow for asking more direct hints. Similarly, when debugging code, first start with asking questions, then providing hints.



might want to make this section structured and display a figure with the entire design space 

how direct vs. indirect to be?


how interactivity helps/helped
one of the differences between chatgpt and codeaid was its interactive features, interactive pseudocode, the relevant function docs, interactive explanations, and etc.


%%%%%%%
support for under-represented groups

%%%%%%%


%%%%%%%
%%%%%%%



%%%%%%%
%%%%%%%
Ask about project/assignment:
Ambiguities in the project description

Educators mentioned this.
However, we did not develop features for this particular use case
But our results show that when we steer the model with prompt engineering, at least, similar to how we did, and other methods, the model can be trusted to not give solutions. 

So for example, future LLM-based tools for education can be populated with both project descriptions, and their solutions.

%%%%%%%
%%%%%%%




\section{Discussion}
The results from our semester-long deployment of CodeAid reveal a promising potential for using LLM-powered coding assistants in educational settings. Students used each of the system's features for a diverse range of inquiry types. Across all system features, the tool was found to have a high degree of helpfulness (86\%), despite not revealing direct code solutions, and many of the improvements made after the midterm feedback were appreciated. Educators echoed many of the benefits identified by students, and particularly, appreciated the pedagogical approach which CodeAid offered. That said, several important concerns and limitations were revealed which will serve as a useful guide for discussion. Below we will discuss the implications for design, future research directions, and limitations of our work.


\subsection{Design Implications}
Based on the findings from our deployment and interviews, we derive the following design implications for future LLM-powered educational tools like CodeAid.

\subsubsection{Mitigating Inaccuracies:}
Given educators' concerns about LLMs potentially misleading students, especially those with weaker fundamentals, it is important that future tools mitigate and/or address inaccuracies. We have identified several possible approaches to this issue.
\begin{enumerate}
    \item \textbf{Provide Better Self-Verification Methods:} Along with LLM-generated answers, CodeAid displays \textbf{verified} documentation for functions relevant to students' queries. As a way to support self-verification, future tools should expand on this by providing more verified resources and instructional material at different granularities, such as course topics, frequently asked questions, sub-goal-labeled worked examples \cite{margulieux2012subgoal}, etc. Additionally, allowing educators to endorse or contribute to these resources could enhance students' trust.
    \item  \textbf{Enhance Transparency:} While disclaimers highlight potential inaccuracies, LLM-based educational tools should embrace a more proactive approach. Our results show that inaccuracies vary across different features or inquiry types. Therefore, displaying recent error statistics, broken down by feature or inquiry type, can help manage user expectations and guide their trust.
    \item \textbf{Aid in Question Formulation:} One reason for inaccuracies can be vague questions with missing context. By helping students frame their questions better, tools can produce more accurate responses. Future tools can utilize LLMs to prompt students to fill in missing details from their queries. In combination, the use of LLM-powered instructional tools designed to help students craft effective prompts may be a promising avenue for future work \cite{denny2023promptly}.
    \item  \textbf{Educate about LLM Limitations:} Experts develop distrust in automated systems when they observe errors \cite{vaithilingam2022expectation}, but students lack the expertise to recognise when outputs are inaccurate and thus could benefit from explicit instruction around model limitations. Before students start using the tool, a tutorial that highlights the strengths and limitations of the LLM can set expectations and discourage over-reliance. This can include exercises where students predict the LLM's accuracy or see varied outputs for the same query.
\end{enumerate}

\subsubsection{Balancing Directness and Helpfulness:}
Educators expressed a preference for keeping introductory programming students in a more controlled environment like CodeAid. However, students frustrated with indirect responses from tools like CodeAid might default to ChatGPT for immediate answers, bypassing the educational safeguards established. Therefore, striking a balance between directness and helpfulness in educational tools becomes crucial to both retain students' engagement and promote deeper understanding. In order to address this, several strategies can be considered:
\begin{enumerate}
    \item \textbf{Differentiating Between Examples and Solutions:} Students expressed that CodeAid sometimes fell short with respect to generating requested code examples, a crucial learning resource \cite{loksa2016role}. Many students from our deployment mentioned they switched to ChatGPT in order to see examples of function usage. However, there is a fine lie with unrestricted LLMs: they can generate tailored examples which might be directly usable solutions. Future iterations of CodeAid should prioritize delivering contextually relevant code that can serve as examples but do not reveal specific solutions.
    \item \textbf{Leverage LLM's Flexibility:} Although pseudo-code was mostly well-received both in our deployment and educator interviews, LLM-generated code can be displayed in other formats. One example is to present generated code in interactive exercises such as Parsons problems, where students have to rearrange code snippets to get the correct solutions \cite{ericson2022parsons}. However, the pedagogical value of such interactions needs further exploration.
    \item \textbf{Gamify the Experience:} Introducing a point system can potentially create a balance between seeking direct solutions and engaging in deeper learning. For example, students could "earn'' the right to ask direct questions by working on interactive exercises (e.g. Parsons problems) generated by the system.
    \item \textbf{Promote Prompt Engineering:} Another opportunity is to teach students about the art of crafting effective prompts, a skill that our interviewed educators emphasized as crucial. From an HCI perspective, this presents a chance to create utilities like template prompt generators for a variety of coding tasks (e.g. debugging, writing or explaining code, etc.) to be used with unrestricted LLMs. These tools can empower students to design their own pedagogical AI Tutors using ChatGPT as proposed by Guo \cite{guo2023opportunities}. Nevertheless, the scalability of this strategy remains questionable, especially as this also necessitates additional training, given the intricacies and unpredictable behaviours of LLMs \cite{zamfirescu2023johnny}.
\end{enumerate}

% \subsection{Future Research Directions}



% \subsubsection{all-encompassing tool:}
% - pedagogical LLM plugins for IDEs: have access to more context from the students' code, students may log-in to courses, opt-in to share their data for personalized help and etc. Such tools might have more adoption, however, it's just a fingertip away from other extensions like Github Copilot which generates code for students and might be determinetal to their learning.

% \subsubsection{providing configurations:}
% - for students: UI, style, font, level of understanding (to an eight year old child), how much information to show, (how in-depth vs. concise),

% to be used in classroom:
% - for educators during a class: more control, what type of response to be produced for different types of asked questions, turn on/off various features
% - monitoring dashboards to assist educators with frequent questions that are being asked, ways for them to dive in and provide contextual feedback to students about their misunderstandings, etc.
% - limit the scope of responses to the topics covered in course (e.g. not showing responses that use complex methods that are out of scope of the class)
% - what if the LLM was aware of the assignments, their complexities.



\subsection{Limitations and Future Research}
Our findings from the deployment of CodeAid are contextualized within a second-year C programming course at a single university, which may not directly generalize to other courses and contexts. Furthermore, the perceived accuracy and utility of CodeAid, which in turn influenced students' trust and engagement, were heavily tied to the OpenAI models we used. The initial release of CodeAid with the `code-davinci-002' model from 2021 could have adversely shaped students' perceptions, particularly when compared to the subsequently adopted GPT-3.5 model from 2023. This factor could explain the some inaccuracies in the tool's performance and the diminishing student engagement we observed. Additionally, the performance of these models varies between different programming languages \cite{xu2022systematic}, or even different code-related tasks (e.g. code explanation, fixing, or generation). In the future, it will also be important to investigate how the use of AI-based coding assistants affects long-term learning outcomes, competency, self-regulation abilities, and frustration levels in educational environments. More controlled studies could also be performed to directly compare these learning outcomes to the use of unrestricted LLMs like ChatGPT.
Finally, as students develop expertise, there may be a time when it would be appropriate to transition from tools like CodeAid to such unrestricted LLMs. Studying the extent of meta-cognitive skills and prompt-crafting abilities needed to prepare for such a transition would be an important area of research. 


\section{Expanding the Scope of CodeAid: Guidelines for Next-Generation LLM-Based Educational Coding Tools}

Drawing from the iterative development of CodeAid and its semester-long deployment, this section presents refined guidelines for the creation of future pedagogical coding assistants powered by large language models (LLMs). These guidelines are informed by the observed student usage patterns (RQ1), the quality of CodeAid's responses (RQ2), student perceptions of CodeAid and ChatGPT (RQ3), and insights from educator interviews (RQ4). The aim is to design LLM-powered tools that provide ethically sound and pedagogically effective assistance, offering scaffolded responses that encourage deep learning without directly providing solutions. We address two primary design challenges that emerged from indirect response generation:

\begin{enumerate}
    \item Enhancing the user-friendliness, predictability, and steerability of tools to ensure that indirect responses are both useful and correct.
    \item Encouraging students to prefer educational AI assistants over direct, productivity-focused alternatives like unmoderated LLMs.
\end{enumerate}

\subsection{Refining Interaction with Indirect AI Responses for Educational Use}

\subsubsection{Facilitating User Engagement with Contextual Clarification and AI Assumptions}
The deployment of CodeAid highlighted a preference among some students for the direct responses of ChatGPT, citing its user-friendliness and perceived learning benefits. This preference is partly due to the ease of verifying direct responses, such as code, compared to the indirect suggestions provided by CodeAid's \textit{Help Fix Code} feature, which were sometimes inaccurate. To counteract this, future LLM-powered educational tools could enhance accuracy by transparently presenting the AI's assumptions and engaging users in refining the AI's understanding. This iterative process not only aids in generating more accurate responses but also promotes educational engagement by encouraging students to consider their inquiries more deeply.

\subsubsection{Increasing Transparency and Predictability in Tool Performance}
To manage expectations and build trust, future educational AI tools should clearly communicate their educational guardrails and how their responses differ from productivity-focused tools. This includes explaining the constraints of the system and offering scaffolded alternatives that encourage self-regulated learning. Providing error statistics by feature or inquiry type can also help users gauge the reliability of the tool and make informed decisions about its use.

\subsubsection{Streamlining Usability with Free-Form Input and Feature Recommendations}
Comparisons with ChatGPT revealed that students found the process of selecting a feature and providing inputs in CodeAid cumbersome. Future tools could improve usability by incorporating a free-form text editor and an AI-powered mechanism to automatically suggest the most relevant system features based on user input. Offering multiple response options for a single input could further enhance the user experience and support learning.

\subsubsection{Employing Direct Scaffolding as a Strategic Approach}
In certain situations, more direct responses may be appropriate. For example, when minor fixes are needed in code debugging, the system could show the corrected code but require the student to engage in an educational activity, such as explaining the reason for the fix. This approach maintains educational engagement while simplifying the verification process.

\subsection{Enhancing Engagement and Preference for Educational AI Over Direct Alternatives}

\subsubsection{Delivering Course-Specific Assistance}
Our findings suggest a preference for AI tools tailored to specific courses, as they provide more targeted responses and allow for assignment-related inquiries. Future tools should integrate course-specific information, such as syllabi, assignments, and lecture notes, to develop unique features that answer course-related questions and align with the students' Zone of Proximal Development.

\subsubsection{Balancing Example Code with Direct Solutions}
While students valued code examples for learning, there is a risk of providing direct solutions. Future tools should differentiate between contextually relevant examples and direct solutions, ensuring that the examples provided do not inadvertently reveal assignment answers.

\subsubsection{Offering Verified Non-AI Resources and Verification Methods}
To enhance trust and predictability, future tools should offer non-AI resources such as instructor-verified materials and internet sources relevant to queries. Features that enable students to perform tasks themselves, such as debugging recipes or code instrumentation, can also support independent learning.

\subsubsection{Creating Interactive and Cognitively Engaging Learning Experiences}
Educators emphasized the importance of cognitive engagement in learning. Future tools should offer varying levels of directness and scaffolding to accommodate different learning preferences and promote deeper cognitive processing. This could include interactive exercises like Parsons problems, where students rearrange code snippets to form correct solutions.

By adhering to these guidelines, future LLM-powered coding assistants can provide valuable educational support that promotes learning, engagement, and ethical use, while remaining a preferred choice over unmoderated direct-response tools.






% # Design Space
% ### Interaction Dynamics:
% - Input Modality and Question Framing: the variety of ways students can pose questions (e.g., natural language, structured formats, code snippets)
% 	- meta-cognition in learning (structuring a question requires students to engage in metacognitive activities, such as self-reflection and self-regulation. By formulating their queries, students are essentially reflecting on their understanding and identifying specific areas of confusion or interest.)
% 	- Inquiry-based learning theories suggest that the process of asking well-formed questions leads to a deeper understanding and promotes critical thinking skills.

% - Interactive Feedback and Verification: the dual responsibility in the learning process: the system's role in adapting and improving based on student interactions, and the student's role in actively engaging with and verifying the information provided
% 	- constructivist theory: as it encourages learners to actively process and contextualize information, rather than passively receiving it.

% - Decision Control on Scaffolding Level: who decides what level of scaffolding is needed (learner autonomy and motivation) what is the instructor's role? the student's preferences? how much agency should the student have? what are the optimal scaffoldings based on ZPD? should it be an adaptive scaffolding? both the system and the AI system contribute to the decision about "what level of scaffolding" when answering a question? what if student's don't find the provided scaffolding level to be suitable for them?
% 	- Theory: Learner autonomy (which refers to the ability of learners to take charge of their own learning process. It emphasizes the role of the learner in setting learning goals, choosing learning strategies, and evaluating their own progress.)

% ### Pedagogical and Ethical Alignment:
% - Scaffolding Method and Directness to improve learning gains: Differentiate between the levels of guidance (e.g., nudges, leading questions, hints, direct explanations, example code, direct and complete solutions) and the method of scaffolding (e.g., gradually increasing complexity, providing partial solutions).
% 	- Theories: Vygotsky's Zone of Proximal Development, Scaffolding theory, Constructivist (students constructing knowledge themselves)

% - balancing academic integrity issues (not displaying solutions) vs. keeping students motivated, engaged


% ### Usage Context and Role:
% - Initiation of Assistance: proactive (assistant-initiated) vs. reactive (student-initiated) exploring the balance between an assistant that initiates help, knows about the students' working context vs. an assistant that only responds to direct queries
% 	- Theories: Self-regulated learning, Inquiry-based learning

% - Role and Context of the Tool (Tool's Position in Learning Ecosystem, Comparison with traditional educational tools)

% - General Purpose vs. Course Specificity

% - Problem-Solving vs. Practice: whether the assistant should focus on solving existing problems or generating new ones for practice, and how this aligns with educational goals.


\begin{itemize}
    \item \textbf{D1 - Student Problem Formulation: Context, Structure, and Initiation:} [[based on X and Y from the study]] In balancing the ease of use and meta-cognitive engagement, this dimension (Figure \ref{fig:design_dimensions} D1) explores how the assistant gathers context (automatically or manually) and the required input format (free-form or structured). The challenge is designing an assistant that is user-friendly yet encourages critical thinking and self-reflection in students. 
    \item \textbf{D2 - Educational Landscape: AI Assistant's Role, Scope, and Advantages:} This dimension defines the role and scope of the AI assistant in relation to other educational resources, like TA office hours. It emphasizes the unique advantages of the assistant and the balance between being a general-purpose tool and one fine-tuned to a specific course. How can AI assistants be designed in a way that ensure students can attain long-lasting skills like prompt engineering, which they may carry forward into their professional lives, while also making sure that safe "guardrails" are enabled to ensure academic integrity within an educational setting. The key trade-offs are achieving versatility without sacrificing educational specificity and balancing productivity-focused with learning-focused and becoming a stepping stone towards a more AI-integrated future.
    \item \textbf{D3 - AI Transparency, User Control, and Feedback Mechanisms:} This dimension deals with the extent of displaying the AI's assumptions on input queries, engaging students in verifying them, and enabling feedback mechanisms to ensure high-quality responses. While increased engagement in the AI's decision-making process and pre-validation (similar to CodeHelp's sufficeny check) can lead to more accurate responses, it may complicate user interaction and potentially overwhelm students. In contrast, post-verification, might be less overwhelming, but less immediate, given the indirect and scaffolded nature of AI responses in educational settings.
    \item \textbf{D4 - Scaffolding, Interactivity, and Learner Autonomy in Responses:} This dimension addresses the directness of responses and the appropriate level of scaffolding that encourages learners to find solutions independently. If the assistant is too direct and students have high autonomy over selecting their desired level of scaffolding, students might miss out on critical learning opportunities tailored to their Zone of Proximal Development. This might negatively impact skill development and self-efficacy. Conversely, too indirect responses, although challenging, can risk discouraging students if they feel overwhelmed, unsupported, and not making progress.
\end{itemize}

------------------------------------------------------------------------------------------------------------------------------------------------------------------------
------------------------------------------------------------------------------------------------------------------------------------------------------------------------
------------------------------------------------------------------------------------------------------------------------------------------------------------------------
------------------------------------------------------------------------------------------------------------------------------------------------------------------------






\subsection{Design Space}
We identified four high-level trade-offs in designing AI-powered educational assistants based on results from our deployment and prior literature.


\textbf{Student Problem Formulation: Context, Structure, and Initiation}

1- how is the assistance initiated? proactive from the assistant in the editor? how do students provide context? structured? free-form? asking the student to ask well-formed questions?
- proactive/reactive (who identifies the source of the problem)
- input format/modality free-form, structured
- 

\textbf{AI Assistant's Role, Scope, and Unique Advantages}

2- how does the AI tool compare to other assistance (AI and non-AI) methods available to students? general-purpose? specific? yet another tool for a course, or just a learning tool, or a tool that they can use forever?
- general purpose, course-specific
- obvious unique values and predictability
- learning-oriented, productivity-focus


\textbf{AI Transparency, Steering, Verification, and Feedback}
4- does the AI system ask for verification before generating the scaffolded, indirect response? (which might be overwhelming) or after it has been generated? and let the student try it? (which might be less predictable)
- pre-verification and clarification might be overwhelming and difficult, while post-verification might be less immediate since scaffolded responses are not direct
- encourage students to not be passive learners, and be critical and reflect on what they learned
- follow-up, feedback (to instructor, to AI),
- wasted time in prompt engineering
- Explainable AI


\textbf{Balancing Scaffolding, Interactivity, and Learner Autonomy}
3- what level of scaffolding should be provided? too direct? how much agency do students have over the level of scaffolding and directness? what's the instructor's role? and the AI system's role?
- student's agency? AI's agency? instructor's?
- level of scaffolding? illusion of capability
- make sure students don't default to unmoderated tools? (ethical, and academic integrity)
- level of interactivity? back-and-forth dialogue? or more direct?
- 

------------------------------------------------------------------------

how much effort should the student go through in order to get assistance when they need? should the system be proactive? should the system allow natural language inputs just as they think about things? or should they formulate their problem in a strict way to encourage deep cognitive engagement?

\textbf{Input Simplicity in Natural Language vs. Strict and Structured Input to Promote Cognitive Engagement}

too far in the spectrum we also have reactive vs. proactive: a student does not even think about their problem, and the system provides some suggestions. but is that good? and should the student identify problems themselves, try to formulate the problem, and learn problem-solving skills?

how the system allows the user to provide input: particularly, how much it focuses on ease of use vs. having the student engage in meta-cognitive activities, such as self-reflection and self-regulation, and asking well-formed questions that promote critical thinking skills? how structured should the input be? vs. completely unstructured.

% how reactive vs proactive should the assistant be? what's the balance? like a plugin that knows what the student is working on and sees if they're struggling and finds a good moment to assist them? vs. a Q/A tool that is initiated by student's asking questions

------------------------------------------------------------------------

what is the AI tool's unique advantages compared to other assistive tools? 
the Tool (Tool's Position in Learning Ecosystem, Comparison with traditional educational tools) 
why should a student use this tool in comparison to other assitive measures? how obvious are the utility of this new tool compared to other tools?

visible and known "added/unique values" compared to other tools?
yet another tool for students to learn how to properly use and master?

how is the AI assistant positioned across the ecosystem of other non-AI assistive and learning tools such as search engines, course content and lecture notes, online Q/A forums, discussion boards, and office hours.

How general-purpose and generic should the AI tool be vs. how specifically should it be to the particular course and educational context that it will be used in? should it be able to handle authentic questions that are outside of the scope of the class? how much detail should it know about the class? assignments? projects? logistics? be able to pull out from topics covered in the class and refer to specific lecture notes?

------------------------------------------------------------------------

\textbf{AI Transparency for Improved Steering vs. Information Overload and Difficult Use}

how transparent should the AI be about itself and what it is doing? how much should it engage the student about its internal processes? how much should the AI system involve the student in verifying these internal processes and asking students to verify and provide feedback to the student to ensure high quality output (rather than just passively receiving it)? how steerable should the AI system be based on feedback from students?

------------------------------------------------------------------------

\textbf{Skill Development vs. Encouraging Progress}
too direct responses and too much autonomy may miss out on critical learning opportunities tailored to their level of Zone of Proximal Development and it might hinder skill development, self-efficacy, .... while too indirect responses (learners need to be challenged to develop confidence) and low autonomy may discourage students. how to ensure progress and maintaing motivation. (self-determination theory) and the importance of experiencing progress and achievement
- what is the appropriate level of scaffolding to use? (e.g., nudges, leading questions, hints, direct explanations, example code, direct and complete solutions) and the method of scaffolding (e.g., gradually increasing complexity, providing partial solutions)
- what is the role of the student? instructor? and the AI? in deciding what level of scaffolding to use? 

------------------------------------------------------------------------

how to keep students engaged, especially in comparison to generic AI tool that are unmoderated --  while at the same time being strict in terms of not showing direct solutions and making sure that students do not over-rely on the tool?

------------------------------------------------------------------------


------------------------------------------------------------------------

(might be a bit too narrow and nuanced)
how broad should the tool be? help generating new problems for practice? help students define 


------------------------------------------------------------------------


------------------------------------------------------------------------


------------------------------------------------------------------------



the Tool (Tool's Position in Learning Ecosystem, Comparison with traditional educational tools) 


in not showing direct solutions? 

how to adhere to academic integrity rules (making sure that students can't cheat by copying direct solutions for summative and graded assessment) and ethical considerations about over-reliance (make sure that students do not over-rely and actually learn from the AI's responses) when students always have the option to use 

balancing academic integrity issues (not displaying solutions) vs. keeping students motivated, engaged

\subsubsection{Assistive Context and Role}


Feedback and Verification

Control and Agency

how do students 


\section{Beyond CodeAid: Implications for Pedagogical LLM-Powered Coding Assistants}
To balance ethical considerations with educational effectiveness, AI assistants liked CodeAid are designed to generate indirect, scaffolded responses. However, our deployment highlighted two major design challenges associated with the nature of indirect responses, especially when these responses might be inaccurate or unhelpful:
\begin{enumerate}
    \item Overall experience may be degraded due to the indirect nature of the responses
    \item students might default to direct tools like ChatGPT
\end{enumerate}

In this section, we draw from the iterative development of CodeAid and insights gained from its semester-long deployment to synthesize guidelines for the design of future LLM-powered educational assistants that would address the above challenges.

\subsection{Optimizing for Ease of Use when Interacting with Indirect AI Tools}

\subsubsection{Engaging the User In Handling Missing Context and Incorrect AI Assumptions}

% validation of correctness becomes less immediate

Our deployment revealed that while some students viewed ChatGPT's direct responses as potentially detrimental to learning, they preferred them over CodeAid's indirect responses for being \textit{user-friendly} and \textit{easier to validate}. For instance in debugging tasks, which made up 32\% of CodeAid's use, students had to manually implement CodeAid's suggestions to check whether the suggestions helped them fix their code. Additionally, inaccurate, misleading, or unhelpful suggestions complicate the process further, leading to trial-and-error and diminished trust in the AI assistant. These inaccuracies are often due to the vagueness of natural language and the incorrect assumptions of the AI about the code and the requested task. Therefore, future tools could enhance accuracy and user trust by adding a \textit{Sufficiency Check} step similar to CodeHelp before generating the final response. This sufficiency check would actively engage users in refining the AI's understanding by prompting users about missing context or clarifying uncertainties. Moreover, this iterative engagement can serve as an educational process, encouraging students to formulate comprehensive questions and thoroughly consider their problems, potentially leading to enhanced learning outcomes.


\subsubsection{Enhancing Usability using Free-Form Input and Automatic Feature Suggestion}~\label{automatic_feature_selection}
Students reported that they appreciated many of CodeAid's interactive features, such as the \textit{Explain Code} feature, which enabled on-hover line-by-line explanations, and the \textit{Help Fix Code} feature, which annotated students' code with fix suggestions. To use these features, students had to choose from one of the five available options and provide input through two input fields. While educators valued this design for promoting active engagement and thoughtful inquiry, students found the process to be cumbersome. This was particularly true when compared to ChatGPT's straightforward, single-input, single-function interface. To enhance usability, future AI assistants could incorporate a free-form text editor with basic syntax highlighting, similar to Markdown, and an AI-powered feature suggestion mechanism that automatically suggests the most relevant system features based on user input, eliminating the need for manual selection. Furthermore, our findings indicate that in some scenarios, students used a variety of different CodeAid features with different inputs to achieve their goals. Future tools can use the LLM to both suggest the top features based on the input inquiry, and tailor the inputs of those features based on the user's query, further removing the burden of manually changing the input to different features. We hypothesize that displaying multiple responses, adapted to the single user input could enhance the user experience and facilitate learning from a variety of perspectives.


\subsubsection{Use More Direct Scaffolding Methods as a Last Resort}
In some scenarios, future AI tools can potentially respond more directly. For example, when students want to debug their code, one of the most frequent use cases of CodeAid, and if the changes (suggested fixes) are minor, then the system can potentially show them the fixed code (and be more direct) however, requiring the students to do some activity such as answering a multiple-choice question about the reason for that fix. Such methods are still using some scaffolding to get the student deeply engaged in the generated solution, but since students see the code, they will potentially be easier to verify. Further research is required to understand how using these scaffolding methods impact learning gains and over-reliance compared to the more indirect approaches used in CodeAid.

% \cite{cockburn2007hard} Hard lessons: Effort-inducing interfaces benefit spatial learning
% can cite: \cite{subramonyam2023bridging} about gulf of execution

% Additionally, employing HCI methods like progressive disclosure \cite{nielsen2006progressive} can enable users to steer the AI more effectively, without information overload, that would lead to more accurate and helpful responses. 

\subsubsection{Transparency and Predictability in Performance and Guardrails}
Furthermore, while disclaimers highlight potential inaccuracies, future LLM-powered educational assistants should take a more proactive approach. Future tools should transparently communicate the implemented guardrails and how responses are tailored to educational settings, instead of focusing on productivity. For instance, when students seek direct code solutions, the system should clearly explain its constraints and offer scaffolded alternatives that promote deeper engagement, emphasizing the importance of self-regulated learning. Furthermore, our results show that inaccuracies vary across different features or inquiry types. Therefore, displaying recent error statistics, broken down by feature or inquiry type, can help manage user expectations and guide their trust.




\subsection{Optimizing for Engagement and Preference over Direct AI Tools}

\subsubsection{Provide Unique, Course-Specific Assistance}
in the spectrum of designing a general-purpose tool vs. a tool that is customized for a specific class and course, results from our deployment of CodeAid are a bit more in favor of designing AI tools that are specific for class since it (a) is able to produce better and more targeted responses, and (b) allows students to ask about project/assignments. this will hopefully helps keep students away from unmoderated tools like ChatGPT,

students found that ChatGPT sometimes produced answers with functions that were not covered in the class, and reported how CodeAid produces responses that are more targeted to the C programming class that students were taking. We argue that this is an important place for future tools to expand on: future AI assistants for educational contexts should pull course-specific information when answering questions as a way to keep students engaged in the tool and make them prefer using it over unmoderated tools like ChatGPT. Future tools can provide mediums for teachers to submit a variety of course-specific information, including assignment and project solutions, course logistics and policies, course syllabus and marking scheme, curriculum outline, as well as lecture notes and course content. This will enable the development of unique features that would help answer students' questions that are specifically about the course, something that generic tools will not be able to do. For example, future tools should help students with their misunderstandings about a project or assignment from their class. Furthermore, by having access to the curriculum, the AI assistants' responses will be more in students' Zone of Proximal development, and therefore, more suitable and appreciated by the students.
With automatic feature selection mentioned in Section \ref{automatic_feature_selection}, a high-level LLM function that serves as a router, will be able to guide students' questions to any of the above information for more accurate and reliable usage. 

% different courses might teach the same content differently, so fine tuning the model on the best practices for this course


\subsubsection{Differentiate Between Example and Direct Solutions}
Students expressed that CodeAid sometimes fell short with respect to generating requested code examples, a crucial learning resource \cite{loksa2016role}. Many students from our deployment mentioned they switched to ChatGPT in order to see examples of function usage. However, there is a fine line with unmoderated LLMs: they can generate tailored examples which might be directly usable solutions. However, our thematic analysis revealed that only 10\% of students' queries were asking for direct code solutions. Many were asking for code and conceptual clarifications, function-specification queries, error message interpretation, and high-level coding guidance. Therefore, unlike CodeAid, future tools should allow delivering contextually relevant code that can serve as examples but do not reveal specific solutions. To ensure that these tools would not reveal assignment and project solutions, future tools that have access to course projects and assignment information can be programmed to refrain from producing code solutions that would be similar to them, instead generate scaffolded alternatives.


\subsubsection{Provide Non-AI Alternatives and Verification Methods}
Some students reported that they lost trust in CodeAid after it did not respond correctly. Another way to improve usability and predictability is by providing non-AI alternatives. CodeAid made one step in this direction by displaying documentations for functions that were relevant to their query... and students found it very useful. Future educational AI tools should expand on this by providing more resources and instructional material at different granularities, such as instructor-verified lecture notes and topics from the course, sub-goal-labeled worked examples \cite{margulieux2012subgoal}, etc. Additionally, allowing educators to endorse or contribute to these resources could enhance students' trust.

Students appreciated CodeAid's ability to offer contextually relevant assistance, mainly because they were able to frame their questions how they think and paste code, something that they were not able to do with search engines. Future tools could expand on this as a non-AI alternative by providing the most relevant internet sources related to their query... which means that responses are less tailored to students' particular queries, but more dependable and easier to verify). 

Moreover, future tools can provide features to help students perform things themselves. For example, for debugging, the tool can provide "debugging recipes" that are contextualized to the task that they're working on. There can also be more active approaches such as injecting instrumentation into students' code so they could understand what is wrong with their code by themselves.

Furthermore, future tools can provide last resorts such as format their question to post on Q/A forums or to format as an e-mail to ask from the professor, as a way to help students be able to easily access the resources that are already available to them through their educational institute.




\subsubsection{Provide Interactive and Cognitively Engaging Scaffolding Methods}
Educators' emphasis on pedagogical soundness (RQ4) suggests that future tools should not only offer correct responses but also promote deeper cognitive processing.

- CodeAid only provided one type of directness for all: pseudo-code. Although it helped students think, but future tools can provide different levels of directness.
%  - what is the appropriate level of directness?
although our deployment did not show the optimal level of scaffolding and directness in the context of our class, however, 

% Our results showed that guardrails can be trusted and when designed properly, can still be engaging and helpful.
% 

%      - promote deeper cognitive engagement

%      - adaptive learning strategies, resonating with the constructivist theory

- varying levels of directness: less direct when students copy task descriptions or directly ask for specific code implementations, compared to when they're asking for what some function does vs. how they can implement this behavior using X vs. how they can use something vs. .even those that reported using ChatGPT, reported that the direct responses generated by ChatGPT were not good for learning. 
- Since some students have strong preferences (e.g. having a personal desirie for self-reliance and solving tasks by themselves) then the system can have some pedagogical settings and customization fields to control: do they want to come up with the solutions themselves, vs. be more direct.
- provide the skeleton of the code, but them fill in the important parts themselves, or help them by asking problem solving questions so that they can come up with the solution themselves.


    % \item \textbf{Leverage LLM's Flexibility:} Although pseudo-code was mostly well-received both in our deployment and educator interviews, LLM-generated code can be displayed in other formats. One example is to present generated code in interactive exercises such as Parsons problems, where students have to rearrange code snippets to get the correct solutions \cite{ericson2022parsons}. However, the pedagogical value of such interactions needs further exploration.




% -  - although identifying the best type of scaffolding is for future research, but we found that students kept using the system even with indirect responses. however, systems can be more direct when students are not asking to generate the entire project/assignment. 
% the need for  of learning which posits that knowledge is actively constructed by the learner based on their experiences and interactions


% \textbf{Improved Trust and Reliability:}
% - each of the suggested features can have a "confidence level" associated to them at two levels: based on the students' query, display what are the unknown assumptions about each method (e.g. if a feature is just prompting them to think about things, then the unknown assumptions are less compared to another feature that is trying to fix the student's code without knowing their entire codebase)
% - if course-specific tools are developed, then the automatic feature suggestion system can also detect which project/assignment students are asking about, and then directing their query to a specific query that knows about that particular project or assignment. as a way to improve accuracy, similar to a TA that is able to better help when they know the solution, they can not only identify what's wrong in a student's code but also provide good hints to them. (below we will talk about the amount of scaffolding and directness) The system is then able to provide scaffolded ways of helping them with much higher accuracy since it has access to the instructor-verified solution, but because of the guardrails, it will never reveal it to the students directly.



% point to CodeHelp also using similar structured input with three input boxes and code language selection. and similarly, pythontutor's new AI assistance, asks the student to decide what they want and they have to provide input, code, and other things int these structured boxes before they can get the final prompt.
% all of this just requires the student to spend a lot of cognitive effort on picking the correct boxes, deciding between features, where to type this and where to type that.

% although educators thought that this help students think before framing their question, and enables an easy and straightforward implementation to ensure high quality responses with different forms of interactive output, but our deployment shows that students that used both ChatGPT and CodeAid prefered ChatGPT's free-form input.





% In summary, to enhance usability and learning efficiency, future tools should incorporate a free-form editor for input, use the LLM to suggest relevant system features based on input, be transparent about the system's guardrails and the assumptions made by the AI, and provide user-friendly interfaces for refining these assumptions to enhance accuracy and educational effectiveness.




- How direct should responses be? What level of scaffolding is appropriate? 
- How can we improve trust and reliability?
- provide non-AI fall-backs when accuracy might be low (such as when trying to help with debugging, the least accurate feature of our system)
- provide verifiable resources and enable self-verification
- allow for customization for different scenarios and use-cases, picking from different scaffolding methods, last resorts

- and eventually, be easy to use (given the complexity of interacting with a blackbox AI model) in terms of providing input, what to expect and predict, and how to steer the AI
    - be transparent: show assumptions, performance history, 
    accuracy, correctness, and helpfulness (so the user does not need to trial-and-error) and be easy to steer and 
    - be easy to navigate
    


From a high-level we can see that educators wanted students to stay in AI tools that were designed with guardrails (knowing that there's a learner using it compared to someone that just wants to maximize productivity). From our end-of-semester survey comparing students' usage of CodeAid with ChatGPT, we found that this requires: ease of use for inputs and steering, course-specific features that provide an added value, higher accuracy, and interactive features.

 and 


Features like General Question and Explain Code were overall more successful, and similarly usages like Asking Programming Questions, Writing and Explaining Code were more accurate, helpful, and received better feedback. However, one of the main use cases with Debugging Code was less accurate, less helpful, and received lower ratings.





% - our results from a real-world deployment show that (1) the majority of students and their queries were not asking for direct code solutions, and (2) many students found the system helpful (although some features were better) and they continued using CodeAid's even though it produced indirect responses 




For more complex usages like debugging, which was one of the main usages of CodeAid, we found that both the first and second iteration of the help-fix-code had low accuracy.










Our v2 system enabled many interactive features in response to students' requests from the first half of the study, however, given the complex nature of how they were implemented with the OpenAI APIs that were available at the time, they required multiple serial LLM calls, which reduced their steerability and transparency (e.g. the user is very limited in terms of how they can steer and navigate the model for example when it has some missing assumptions or something else).

Future tools, can utilize the powerful capabilities of GPT-4 that follows provided templates to create domain-specific languages (DSLs) \cite{ym2023pwr} be designed with GPT-4's DSL support and report back any "guesses" that they're making and assumptions that they're having when.





\textbf{Interactive Features}





This is the most certain thing that we learned -- it optimizes multiple things:

- makes sure that responses are in students' zone of proximal development, increasing learning effectiveness
- promotes self-verification, so students
- it helps students stay in these "approved" tools that have these "guardrails" instead of defaulting to ChatGPT
-  


- providing more course-specific material
- general purpose vs. specific class

we have evidence from the interviews and weekly surveys that show how students liked and felt that the tool is targeted more towards C programming compared to ChatGPT and other tools... so future tools: the more students understand that the tool is tailored specifically to their course, their assignments, their projects, they will use it more for the class.
- ask about projects/assignments
[any other ways to attract students to keep in the tool?]




Pedagogical:
Provide Varying levels of scaffolding

Educators' emphasis on pedagogical soundness (RQ4) suggest that future tools should promote deeper cognitive processing. 

The variability in students' usage patterns (RQ1) the need for adaptive strategies, resonating with the constructivist theory of learning with posits that knowledge is actively constructed by the learner based on their experiences and interactions.

- Scaffolding method: promote critical thinking, problem-solving, and self-reflection.







Our results from deploying CodeAid 
- understand how students will use such a tool in a semester-long deployment, what types of questions they will ask, how they use this tool in comparison to other available tools that they have (office hours), and what new unique interactions and usages it will enable. whether it will help scale up instruction and help under-represented groups?
- we then tried to understand what did students think of the LLM's responses? and how did we (the researchers) evaluate the responses in terms of correctness, helpfulness, and directly revealing code solutions. we frequently asked students why they used or not used the system, and how it helped them?
- at the end of the course, we asked students to compare CodeAid with ChatGPT. This helped us see which parts of our results could be generalized, which parts are related to the interaction, and where did CodeAid do better, and where did ChatGPT do better.
- Finally, we conducted eight interviews with educators that serves as a great bridge from CodeAid to beyond CodeAid and the implications for future LLM-powered coding assistants.
- This section aims to extend the discussion beyond CodeAid, using our findings as a foundation to inform the design of future LLM-Powered Coding Assistants specifically tailored for learning environments.

% A summary of what we found:
Our semester-long deployment of CodeAid 
- our thematic analysis of ~1750 queries asked from CodeAid using the five features that we developed, helped us identify four categories and nine subcategories of different types of queries and their frequency/proportions.
- we found that 79\% of responses were correct, and 67\% were helpful. We also identified reasons for when students rated queries high or poorly for each of the features. In terms of directly revealing code solutions, X\% were only in natural language, Y\% included high-level pseudocode, Z\% included specific pseudocode, N\% included 
- support for under-represented groups: females used the system more compared to males, and 
- 

------------------------------------------------------------------------------------------------------------



adapting to learner's zone of proximal development (Vygotsky’s):
- LLMs can act as a more knowledgeable other... adaptive responses cater to individual learning needs... some students wanted to explain things "like an eight year old" or they really liked how they could ask many questions without being judged... 

Promoting Critical Thinking... ask probing questions or offer guidance that leads students to discover solutions themselves, rather than providing direct answers.

constructivist learning principles, where knowledge is actively constructed by the learner... aligning with Piaget’s theory of cognitive development.

% The variability in students' usage patterns (RQ1) underscores the need for adaptive learning strategies, resonating with the constructivist theory of learning which posits that knowledge is actively constructed by the learner based on their experiences and interactions (Piaget, 1954). Future LLM-powered tools should personalize learning paths, adapting to individual student's inquiry types and frequencies, thereby facilitating a more tailored and effective learning experience. This aligns with Vygotsky's (1978) zone of proximal development, suggesting that tools should provide scaffolding adjusted to the learner's current level of understanding.


% \subsubsection{Enhanced Pedagogical Approach}
%  This aligns with Mayer’s Cognitive Theory of Multimedia Learning, which advocates for designing educational experiences that optimize cognitive processing. Tools should encourage critical thinking and problem-solving skills, reflecting Bloom's Taxonomy, by guiding students through the problem-solving process rather than providing direct solutions.


% \subsubsection{Student Engagement and Interactive Learning}
% The request for more interactive features like code execution (RQ4) and high usage of interactive features in CodeAid (RQ1) point towards the need for more engaging and interactive learning experiences. According to Malone's Theory of Intrinsically Motivating Instruction, such features can enhance curiosity and control, key elements for engaging learning experiences. Interactive exercises, aligned with experiential learning theory (Kolb, 1984), can provide hands-on learning opportunities, enhancing understanding and retention.


% \subsubsection{Customization and Control for Educators}
% Educators' desire for customizable responses (RQ4) suggests that future tools should allow instructors to tailor the tool’s behavior to align with their pedagogical goals and course content. This is consistent with the concept of Technological Pedagogical Content Knowledge (TPACK), which emphasizes the intersection of technology, pedagogy, and content in effective teaching. Educators should be able to configure the tool to vary the level of guidance based on the course level and learning objectives.


% \subsubsection{Monitoring and Analytics}
% The suggestion for monitoring dashboards (RQ4) aligns with the need for formative assessment tools in education, as posited by Black and Wiliam (1998). These dashboards can provide educators with insights into student learning processes, helping identify common misunderstandings and adjust teaching strategies accordingly. However, this should be balanced with considerations of privacy and student autonomy.



different levels of optimization:
students liked the interactive features of CodeAid, such as the line-by-line explanations of the pseudocode. however, both educators and students found 
- direct vs. indirect -> dynamically deciding: code vs. pseudocode vs. some other indirect method (e.g. making the user think about the task) (Differentiating Between Examples and Solutions)



Single Text Input with AI-Suggested Responses and Alternatives:
- ease of use and learning? In comparison to ChatGPT, students wanted an easier way to interact with the system.... interactive features of CodeAid were fine... the problem was with how they needed to specify the action and do many clicks. so future tools should 


our results, including the dataset of questions asked by students that we made public, help develop future tools by understanding what types of questions students asked. which means we 

- if they didn't like the responses, then it should provide alternatives. this could also reduce the chance of switching to unguraded tools like ChatGPT

similar to bing chat's references, CodeAid's relevant function documentations was highly favored by the students from our deployment. future tools can improve this for several reasons:
- improved self-verification
- provide more learning opportunities
this can also be extended by tools similar to Bing Chat that provide sources from around the web (e.g. w3schools, wikipedia, etc.)


Reasons to Keep Students in the tool:


if a student does not trust codeaid, provide prompt builders, so that they'd at least have the chance to use chatgpt with guardrails... guardrails that they could edit themselves if needed.

Future tools should be designed to provide various AI and non-AI alternatives
non-AI can be:
- using the LLM to convert the student's question to a proper Stackoverflow question so they can ask there, or something that they can post on the Q/A forum of their class


% excited about AI: scaling up instruction + mimicing what an expert instructor would do
% Expected general design guidelines for the design of classroom tools using LLMs -> people designing classroom tools using LLMs 
% general design principles for LLM-based coding tools
% broader insights” that inform the design of LLM-powered coding assistants
% critical discussion of how answers to set RQs could have an impact on future design and adoption of digital TA  
% Is it possible to make a system that optimizes for both learning and ease-of-use? Or is this a fundamental tradeoff in the design of LLM-based educational tools?


Unlike CodeAid that provided similar levels of directness to all queries, future tools should be able to provide a customized 



Future classroom assistants should provide different levels of directness for different types of asked queries.
If students request for direct code solutions (which was 10\% of the questions asked), the system should work as a guiding TA. At first asking self-reflecting questions so they can think more deeply about the task and if that was not enough, allow for asking more direct hints. Similarly, when debugging code, first start with asking questions, then providing hints.



might want to make this section structured and display a figure with the entire design space 

how direct vs. indirect to be?


how interactivity helps/helped
one of the differences between chatgpt and codeaid was its interactive features, interactive pseudocode, the relevant function docs, interactive explanations, and etc.


%%%%%%%
support for under-represented groups

%%%%%%%


%%%%%%%
%%%%%%%



%%%%%%%
%%%%%%%
Ask about project/assignment:
Ambiguities in the project description

Educators mentioned this.
However, we did not develop features for this particular use case
But our results show that when we steer the model with prompt engineering, at least, similar to how we did, and other methods, the model can be trusted to not give solutions. 

So for example, future LLM-based tools for education can be populated with both project descriptions, and their solutions.

%%%%%%%
%%%%%%%




\section{Discussion}
The results from our semester-long deployment of CodeAid reveal a promising potential for using LLM-powered coding assistants in educational settings. Students used each of the system's features for a diverse range of inquiry types. Across all system features, the tool was found to have a high degree of helpfulness (86\%), despite not revealing direct code solutions, and many of the improvements made after the midterm feedback were appreciated. Educators echoed many of the benefits identified by students, and particularly, appreciated the pedagogical approach which CodeAid offered. That said, several important concerns and limitations were revealed which will serve as a useful guide for discussion. Below we will discuss the implications for design, future research directions, and limitations of our work.


\subsection{Design Implications}
Based on the findings from our deployment and interviews, we derive the following design implications for future LLM-powered educational tools like CodeAid.

\subsubsection{Mitigating Inaccuracies:}
Given educators' concerns about LLMs potentially misleading students, especially those with weaker fundamentals, it is important that future tools mitigate and/or address inaccuracies. We have identified several possible approaches to this issue.
\begin{enumerate}
    \item \textbf{Provide Better Self-Verification Methods:} Along with LLM-generated answers, CodeAid displays \textbf{verified} documentation for functions relevant to students' queries. As a way to support self-verification, future tools should expand on this by providing more verified resources and instructional material at different granularities, such as course topics, frequently asked questions, sub-goal-labeled worked examples \cite{margulieux2012subgoal}, etc. Additionally, allowing educators to endorse or contribute to these resources could enhance students' trust.
    \item  \textbf{Enhance Transparency:} While disclaimers highlight potential inaccuracies, LLM-based educational tools should embrace a more proactive approach. Our results show that inaccuracies vary across different features or inquiry types. Therefore, displaying recent error statistics, broken down by feature or inquiry type, can help manage user expectations and guide their trust.
    \item \textbf{Aid in Question Formulation:} One reason for inaccuracies can be vague questions with missing context. By helping students frame their questions better, tools can produce more accurate responses. Future tools can utilize LLMs to prompt students to fill in missing details from their queries. In combination, the use of LLM-powered instructional tools designed to help students craft effective prompts may be a promising avenue for future work \cite{denny2023promptly}.
    \item  \textbf{Educate about LLM Limitations:} Experts develop distrust in automated systems when they observe errors \cite{vaithilingam2022expectation}, but students lack the expertise to recognise when outputs are inaccurate and thus could benefit from explicit instruction around model limitations. Before students start using the tool, a tutorial that highlights the strengths and limitations of the LLM can set expectations and discourage over-reliance. This can include exercises where students predict the LLM's accuracy or see varied outputs for the same query.
\end{enumerate}

\subsubsection{Balancing Directness and Helpfulness:}
Educators expressed a preference for keeping introductory programming students in a more controlled environment like CodeAid. However, students frustrated with indirect responses from tools like CodeAid might default to ChatGPT for immediate answers, bypassing the educational safeguards established. Therefore, striking a balance between directness and helpfulness in educational tools becomes crucial to both retain students' engagement and promote deeper understanding. In order to address this, several strategies can be considered:
\begin{enumerate}
    \item \textbf{Differentiating Between Examples and Solutions:} Students expressed that CodeAid sometimes fell short with respect to generating requested code examples, a crucial learning resource \cite{loksa2016role}. Many students from our deployment mentioned they switched to ChatGPT in order to see examples of function usage. However, there is a fine lie with unrestricted LLMs: they can generate tailored examples which might be directly usable solutions. Future iterations of CodeAid should prioritize delivering contextually relevant code that can serve as examples but do not reveal specific solutions.
    \item \textbf{Leverage LLM's Flexibility:} Although pseudo-code was mostly well-received both in our deployment and educator interviews, LLM-generated code can be displayed in other formats. One example is to present generated code in interactive exercises such as Parsons problems, where students have to rearrange code snippets to get the correct solutions \cite{ericson2022parsons}. However, the pedagogical value of such interactions needs further exploration.
    \item \textbf{Gamify the Experience:} Introducing a point system can potentially create a balance between seeking direct solutions and engaging in deeper learning. For example, students could "earn'' the right to ask direct questions by working on interactive exercises (e.g. Parsons problems) generated by the system.
    \item \textbf{Promote Prompt Engineering:} Another opportunity is to teach students about the art of crafting effective prompts, a skill that our interviewed educators emphasized as crucial. From an HCI perspective, this presents a chance to create utilities like template prompt generators for a variety of coding tasks (e.g. debugging, writing or explaining code, etc.) to be used with unrestricted LLMs. These tools can empower students to design their own pedagogical AI Tutors using ChatGPT as proposed by Guo \cite{guo2023opportunities}. Nevertheless, the scalability of this strategy remains questionable, especially as this also necessitates additional training, given the intricacies and unpredictable behaviours of LLMs \cite{zamfirescu2023johnny}.
\end{enumerate}

% \subsection{Future Research Directions}



% \subsubsection{all-encompassing tool:}
% - pedagogical LLM plugins for IDEs: have access to more context from the students' code, students may log-in to courses, opt-in to share their data for personalized help and etc. Such tools might have more adoption, however, it's just a fingertip away from other extensions like Github Copilot which generates code for students and might be determinetal to their learning.

% \subsubsection{providing configurations:}
% - for students: UI, style, font, level of understanding (to an eight year old child), how much information to show, (how in-depth vs. concise),

% to be used in classroom:
% - for educators during a class: more control, what type of response to be produced for different types of asked questions, turn on/off various features
% - monitoring dashboards to assist educators with frequent questions that are being asked, ways for them to dive in and provide contextual feedback to students about their misunderstandings, etc.
% - limit the scope of responses to the topics covered in course (e.g. not showing responses that use complex methods that are out of scope of the class)
% - what if the LLM was aware of the assignments, their complexities.



\subsection{Limitations and Future Research}
Our findings from the deployment of CodeAid are contextualized within a second-year C programming course at a single university, which may not directly generalize to other courses and contexts. Furthermore, the perceived accuracy and utility of CodeAid, which in turn influenced students' trust and engagement, were heavily tied to the OpenAI models we used. The initial release of CodeAid with the `code-davinci-002' model from 2021 could have adversely shaped students' perceptions, particularly when compared to the subsequently adopted GPT-3.5 model from 2023. This factor could explain the some inaccuracies in the tool's performance and the diminishing student engagement we observed. Additionally, the performance of these models varies between different programming languages \cite{xu2022systematic}, or even different code-related tasks (e.g. code explanation, fixing, or generation). In the future, it will also be important to investigate how the use of AI-based coding assistants affects long-term learning outcomes, competency, self-regulation abilities, and frustration levels in educational environments. More controlled studies could also be performed to directly compare these learning outcomes to the use of unrestricted LLMs like ChatGPT.
Finally, as students develop expertise, there may be a time when it would be appropriate to transition from tools like CodeAid to such unrestricted LLMs. Studying the extent of meta-cognitive skills and prompt-crafting abilities needed to prepare for such a transition would be an important area of research. 



----------
----------
----------
----------
----------

\section{Beyond CodeAid: Implications for Pedagogical LLM-Powered Coding Assistants}
This section draws from the iterative development of CodeAid and insights gained from its semester-long deployment to derive broader implications for the design of AI assistants in educational contexts. Our results point to four high-level dimensions within the emerging design space, each with unique usability and educational trade-offs. These dimensions include: \textbf{(D1)} \textit{Student Problem Formulation: Context, Structure, and Initiation}, \textbf{(D2)} \textit{Educational Landscape: AI Assistant's Role, Scope, and Unique Advantages}, \textbf{(D3)} \textit{AI Transparency, User Control, and Feedback Mechanisms}, and \textbf{(D4)} \textit{Scaffolding, Interactivity, and Learner Autonomy in Responses}.

% given the compelx nature of the design space, 

For each dimension (presented in Figure~ ~\ref{fig:design_dimensions}) we will first highlight the relevant aspects of our findings that point to it. We will then delve into discussing the key questions and design decisions, along with educational and usability trade-offs associated with that dimension. Lastly, we will synthesize implications and guidelines for designing future educational AI assistants, aiming to address some of these identified trade-offs.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{sections/figures/design-dimensions.png}
    \caption{Emerging dimensions and trade-offs within the design space of AI-powered assistants for educational contexts}
    \label{fig:design_dimensions}
\end{figure}

\subsection{D1 - Student Problem Formulation: Context, Structure, and Initiation}
When using CodeAid, students found its feature selection UI complex and that its structured input fields limited how they should ask questions and provide context. Conversely, students that used both CodeAid and ChatGPT, preferred ChatGPT for its single, free-form input interface. Educators appreciated CodeAid's design, which involved selecting from five options and providing structured inputs. They found that it promoted active engagement, critical thinking, and thoughtful inquiry. Furthermore, in terms of providing context to the AI, some students desired more efficient interactions by allowing the AI to have access to their entire code. Similarly, others observed that CodeAid was unable to debug effectively without having access to their entire program.

% Additionally, our usage patterns indicate that in situations like debugging code, students used a variety of CodeAid features in combination. % Furthermore, our findings indicate that in some scenarios, students used a variety of different CodeAid features with different inputs to achieve their goals. some features might have been less useful for some scenarios. 

This leads to the first dimension in the design space: balancing between students' ease of use and their meta-cognitive engagement when asking questions from the assistant (Figure \ref{fig:design_dimensions} D1). This dimension explores (a) whether the assistant automatically gathers context (like a plugin in an IDE) or requires manual input from the user, (b) whether the assistant allows students to ask questions in a manner, similar to how they think, or requires input in a specific structure and format, and (c) the assistant's level of reactivity versus proactivity in identifying problems and facilitating help-seeking. The trade-offs include that automatic context integration, free-form input methods, and proactive assistance may enhance usability and ease of use, but could potentially reduce opportunities for students to engage in meta-cognitive activities such as self-reflection and asking well-formed questions that promote critical thinking.

To enhance usability, future AI assistants can incorporate a free-form text editor with basic syntax highlighting, similar to MarkDown, to provide \textit{optional} structure. However, considering that students may ask vague questions with insufficient context, future tools could use the AI to display a restructured version of their queries back to students and encourage them to reflect on it. Furthermore, to eliminate manual selection of features, future tools can use the AI to recommend the most relevant system features based on the user's input. We hypothesize that displaying multiple responses, adapted to the single user input could enhance the user experience and facilitate learning from a variety of perspectives. 

Future research is needed to evaluate the impact of proactive problem identification and assistance in education, focusing on potential student over-reliance and the design of minimally distracting assistants, similar to the considerations for tools like GitHub Copilot \cite{mozannar2022reading}.






\subsection{D2 - Educational Landscape: AI Assistant's Role, Scope, and Unique Advantages}
Some students from our study highlighted benefits shared between CodeAid and ChatGPT which were not present in non-AI tools like search engines. These included the ability to interact with the tool in natural language, contextual assistance, and the AI's tailored responses. In contrast, other students pinpointed unique advantages in CodeAid, such as its stimulation of critical thinking (using pseudo-code), technical focus on C programming (relevant to their course), and its capability to "pull" comprehensive documentation related to queries. Furthermore, educators showed a strong preference for students using learner-focused AI tools like CodeAid over more generic productivity tools like ChatGPT, to uphold academic integrity and promote effective learning. They recommended integrating these tools into code editors for easier access and higher engagement. On a different note, some students expressed a desire to learn more effective ways of writing prompts, considering it a vital skill. However, due to the educational focus of such LLM-based assistants, incorporating this feature might not align with the scope of the tool.

This leads to the second dimension in the design space: determining the role, scope, and unique advantages of future educational AI assistants in relation to other educational resources, like TA office hours (Figure \ref{fig:design_dimensions} D2). It emphasizes the unique advantages of the assistant and the balance between being a general-purpose tool and one fine-tuned to a specific course. How can AI assistants be designed to ensure students develop long-lasting skills such as prompt engineering, skills they may carry forward into their professional lives? Additionally, it's crucial to make sure that safe 'guardrails' are enabled to maintain academic integrity within an educational setting. Overall, the key trade-offs are achieving versatility without sacrificing educational specificity and balancing productivity-focused with learning-focused and becoming a stepping stone towards a more AI-integrated future.

Considering the rapidly expanding ecosystem of productivity-focused AI tools, it is challenging to keep students in a learner-centric AI tool. To address this issue, our results suggest designing course-specific AI assistants. These assistants should be capable of (a) generating accurate, technically correct, and informative responses, including references to specific lecture notes, and (b) allowing students to ask detailed questions about their course projects, assignments, and logistics. Furthermore, with access to the curriculum, the AI assistants' responses will align more closely with students' Zone of Proximal Development, making them more relevant and beneficial for the students. These tools can also instructor-verified content

Moreover, considering the natural language processing capabilities of LLMs and how they provide contextualized assistance, future tools have the potential to broaden their scope by serving as gateways to non-AI content and resources. CodeAid has already taken a step in this direction by displaying relevant function documentations, which students greatly appreciated. Future educational AI tools could further enhance this by retrieving relevant StackOverflow posts, similar to Bing Chat, as well as providing access to instructor-verified practice exercises and sub-goal-labeled worked examples \cite{margulieux2012subgoal}. 

% Additionally, future tools could offer 'debugging recipes' tailored to the students' inputs, enabling them to inject instrumentation code into their work for independent debugging. Finally, these tools could act as a last resort by assisting students in formatting their questions for posting on Q\&A forums, thereby facilitating easy access to the plethora of resources available through their educational institutions.






\subsection{D3 - AI Transparency, User Control, and Feedback Mechanisms}
The low transparency and predictability of AI tools are fundamental issues in modern generative AI models. However, these challenges are compounded in educational AI assistants, which are designed to provide scaffolded, indirect responses without directly revealing solutions. For instance, CodeAid typically generated natural language suggestions to assist with debugging, or provided pseudo-code to assist with writing code. Our thematic analysis showed how these responses were sometimes incorrect or unhelpful. We found that students seeking to verify CodeAid's responses often had to write and test a small program based on the provided suggestions. In contrast, students using ChatGPT could directly access and run the generated code for verification. Furthermore, when responses were incorrect or not helpful, students often asked follow-up questions, asked a new question with slightly modified prompt, or even retried with the same prompt. This unpredictability and difficulty in steering the AI, coupled with a trial-and-error approach, eroded trust in the AI assistant. As a result, some students stopped using CodeAid or ChatGPT entirely, while others shifted to ChatGPT, preferring its more direct response style for easier trial-and-error processes.

This points to the third dimension in our design space: considering the indirect nature of responses in educational AI assistants, how can we maximize user-experience, efficiency, and predictability of obtaining a helpful response (Figure \ref{fig:design_dimensions} D3). This dimension explores the extent of displaying the AI's assumptions on input queries, engaging students in verifying them, and enabling feedback mechanisms to ensure high-quality responses. While increased engagement in steering and validating the AI's assumptions before generating a response can lead to higher accuracy, it may complicate user interaction and potentially overwhelm students. In contrast, validating the response after generation might be less overwhelming, but less immediate, given its indirect and scaffolded nature in educational settings.

Although this needs further research, but future tools could enhance accuracy and user trust by adding a \textit{Sufficiency Check} step similar to CodeHelp \cite{liffiton2023codehelp} before generating the final response. This sufficiency check would actively engage users in refining the AI's understanding by prompting users about missing context or clarifying uncertainties. Moreover, this iterative engagement can serve as an educational process, encouraging students to formulate comprehensive questions and thoroughly consider their problems, potentially leading to enhanced learning outcomes.

Moreover, future tools could enhance the validation of scaffolded responses by including code execution capabilities and enabling users to interact with and test the underlying code generated by the AI, without directly revealing it. This interaction could be facilitated through a line-by-line execution interface, similar to PythonTutor \cite{guo2013online}, and can use a black-box approach or represent a pseudo-code version.






\subsection{D4 - Scaffolding, Interactivity, and Learner Autonomy in Responses}
Students and educators had diverse views and requirements regarding the level of directness and scaffolding an AI assistant should offer. Students exhibited varying needs: some sought explicit example codes, others preferred subtle hints, and there were instances where they simply wanted the AI to provide direct solutions. Similarly, educators observed that in certain scenarios, the use of self-reflective questions could encourage students to independently solve problems, while in other scenarios, they noted that excessive scaffolding could lead to frustration. Furthermore, educators highlighted the importance of customization options, allowing them to tailor the AI's level of assistance, such as restricting the display of pseudo-code for specific queries or during certain course segments, to better align with pedagogical goals.

This introduces the fourth dimension in the evolving design space: finding the right balance between sufficient scaffolding for critical learning and minimizing frustration, while also considering the degree of autonomy learners should have in personalizing their scaffolding experience (Figure \ref{fig:design_dimensions} D4). If the assistant is too direct and students have high autonomy over selecting their desired level of scaffolding, students might miss out on critical learning opportunities tailored to their Zone of Proximal Development. This might negatively impact skill development and self-efficacy. Conversely, too indirect responses, although challenging, can risk discouraging students if they feel overwhelmed, unsupported, and not making progress.

To promote deeper cognitive engagement and ensuring progress, future tools might, as a last resort, display generated code but lock the AI tool until students complete a specific learning activity. This could involve the AI assistant highlighting critical sections of the code and prompting students to answer questions about these parts. Additionally, future AI tools could foster independent problem-solving using the Socratic Method \cite{tamang2021comparative} and transforming code generation requests into a series of problem-solving questions. With each correct response, the tool would reveal the code segment corresponding to that question. 

Furthermore, since code examples are a crucial learning resource \cite{loksa2016role}, future AI assistants can differentiate between example code and direct solutions. Our thematic analysis revealed that a majority of queries were asking for code and conceptual clarifications, function-specification queries, error message interpretation, and high-level coding guidance. Consequently, future tools could be designed more leniently and display example codes in response to these types of queries.

